Regression adjustments for estimating the global treatment effect in experiments with interference

Standard estimators of the global average treatment effect can be biased in the presence of interference. This paper proposes regression adjustment estimators for removing bias due to interference in Bernoulli randomized experiments. We use a fitted model to predict the counterfactual outcomes of global control and global treatment. Our work differs from standard regression adjustments in that the adjustment variables are constructed from functions of the treatment assignment vector, and that we allow the researcher to use a collection of any functions correlated with the response, turning the problem of detecting interference into a feature engineering problem. We characterize the distribution of the proposed estimator in a linear model setting and connect the results to the standard theory of regression adjustments under SUTVA. We then propose an estimator that allows for flexible machine learning estimators to be used for fitting a nonlinear interference functional form. We propose conducting statistical inference via bootstrap and resampling methods, which allow us to sidestep the complicated dependences implied by interference and instead rely on empirical covariance structures. Such variance estimation relies on an exogeneity assumption akin to the standard unconfoundedness assumption invoked in observational studies. In simulation experiments, our methods are better at debiasing estimates than existing inverse propensity weighted estimators based on neighborhood exposure modeling. We use our method to reanalyze an experiment concerning weather insurance adoption conducted on a collection of villages in rural China.

==> macros.tex <==
\usepackage{amsmath,amsthm,amssymb,eurosym}
\usepackage{enumerate}
\usepackage{graphicx}
%\usepackage{cite}
\usepackage{fancyhdr}
\usepackage{lastpage}
\usepackage{titlesec}
\usepackage[OT2,T1]{fontenc} 
\usepackage[russian,american]{babel} 
\usepackage{lastpage}
\usepackage{float}
\usepackage{bbm}
\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{color}
\usepackage{soul} %for highlighting
\usepackage{wrapfig}
\usepackage{verbatim}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{framed} % for shaded boxes

\usepackage{url}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{subcaption}
\usepackage{hyperref}

\usepackage[utf8]{inputenc}
\usepackage{csquotes} % for block quotes


%~~~~~~~~~~~~~~~~
% Commonly Used Letters
%~~~~~~~~~~~~~~~~
\newcommand{\R}{\mathbb{R}} 	% real numbers	
%\newcommand{\C}{\mathbb{C}} 	% complex numbers	
\newcommand{\Z}{\mathbb{Z}} 	% integers
\newcommand{\Q}{\mathbb{Q}} 	% rational numbers
\newcommand{\N}{\mathbb{N}} 	% natural numbers	



\renewcommand{\P}{\mathbf{P}} 	% probability
\newcommand{\E}{\mathbf{E}} 	% expectation
\newcommand{\V}{\mathbf{V}} 	% variance
\newcommand{\bias}{\operatorname{Bias}}   % bias
\newcommand{\var}{\operatorname{Var}}   % variance
\newcommand{\Var}{\operatorname{Var}}   % variance
\newcommand{\cov}{\operatorname{Cov}} 	% covariance
\newcommand{\Cov}{\operatorname{Cov}}   % covariance
\newcommand{\Corr}{\operatorname{Corr}} % correlation

%~~~~~~~~~~~~~~~~
% Calligraphic Letters
%~~~~~~~~~~~~~~~~
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cZ}{\mathcal{Z}}
\newcommand{\cW}{\mathcal{W}}
%~~~~~~~~~~~~~~~~
% Blackboard or Bold Letters
%~~~~~~~~~~~~~~~~
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\I}{\mathbb{bI}} 	% indicator variable
\newcommand{\one}{\mathbbm{1}} 	% indicator variable
\renewcommand{\S}{\mathbb{bS}}
\newcommand{\bW}{\mathbb{W}}
\newcommand{\bV}{\mathbb{V}}

%~~~~~~~~~~~~~~~
% Distributions
%~~~~~~~~~~~~~~~
\def\Gsn{\mathcal{N}}
\def\ber{\textnormal{Ber}}
\def\bin{\textnormal{Bin}}
\def\unif{\textnormal{Unif}}
\def\mult{\textnormal{Mult}}
\def\NegMult{\textnormal{NegMult}}
\def\Dir{\textnormal{Dir}}
\def\bet{\textnormal{Beta}}
\def\pois{\textnormal{Pois}}
\def\HypGeo{\textnormal{HypGeo}}
\def\GEM{\textnormal{GEM}}
\def\BP{\textnormal{BP}}
\def\DP{\textnormal{DP}}
\def\BeP{\textnormal{BeP}}
\def\Exp{\textnormal{Exp}}
\def\gam{\textnormal{Gamma}}

\newcommand{\vect}[1]{\mathbf{#1}}
\newcommand{\+}[1]{\mathbf{#1}}
\newcommand{\vectsym}[1]{\boldsymbol{#1}}


\newcommand{\ip}[2]{\left \langle #1, #2 \right\rangle}
\newcommand{\norm}[1]{\left \lVert #1 \right \rVert}
\newcommand{\abs}[1]{\left \lvert #1 \right \rvert}

\newcommand{\ds}{\displaystyle}
\newcommand{\ep}{\varepsilon}

\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\newcommand{\argmax}{\operatornamewithlimits{argmax}}
%\DeclareMathOperator*{\argmin}{arg\,min}
%\DeclareMathOperator*{\argmax}{arg\,max}
\newcommand{\on}[1]{\operatorname{#1}}

\newcommand{\tr}{\on{tr}} % trace

%~~~~~~~~~~~~~~~~
% Some abbreviations
%~~~~~~~~~~~~~~~~
\newcommand{\plim}{\stackrel{P}{\to}} % convergence in probability
\newcommand{\pto}{\stackrel{p}{\to}}
\newcommand{\wlim}{\Rightarrow} % weak convergence
\newcommand{\wto}{\Rightarrow}
\newcommand{\asto}{\stackrel{\text{a.s.}}{\to}} %a.s. convergence
\newcommand{\lpto}[1]{\stackrel{L^#1}{\to}} %L^p convergence


\newcommand{\io}{\text{ i.o.}} 	%infinitely often
\newcommand{\fo}{\text{ f.o.}} 	%infinitely often
\newcommand{\pderiv}[1]{\frac{\partial}{\partial #1}}	%partial derivative
\newcommand{\equaldist}{\stackrel{\mathcal{D}}{=}}  %equal in distribution
\newcommand{\eqlaw}{\stackrel{\mathcal{L}}{=}} %equal in law
%
\newcommand{\defeq}{\stackrel{\text{def}}{=}}  %define something
\newcommand{\seteq}{\stackrel{\text{set}}{=}}  %define something
%
\newcommand{\iid}{\stackrel{\text{iid}}{\sim}} % independent and identically distributed
\newcommand{\ind}{\stackrel{\text{ind}}{\sim}} % just independent
%

% Playing with colors
\newcommand{\need}[1]{\textcolor{red}{#1}}
\newcommand{\notate}[1]{\textcolor{red}{\textbf{[#1]}}}
\newcommand{\note}[1]{\textcolor{red}{\textbf{[#1]}}}
\newcommand{\highlight}[1]{\colorbox{yellow}{#1}}
\newcommand{\colorparagraph}[1]{\paragraph{\colorbox{YellowOrange}{#1}}}
\newcommand{\sectionhead}[1]{\begin{center}\colorbox{LimeGreen}{\textsc{\textbf{#1}}}\vspace{-2ex}\end{center}}



% Shaded box settings
\definecolor{shadecolor}{rgb}{1,0.9,0.8} % set color
\newcommand{\caution}[1]{
	\begin{shaded}
	\vspace{-18pt}
	\paragraph{Caution: }
	#1
	\end{shaded}
	}

% Defining problem and solution
\newcommand{\prob}[1]{\paragraph{#1.}}
\newcommand{\ques}{\paragraph{Question.}}
\newcommand{\sol}{\begin{proof}[Solution.]}
\newcommand{\esol}{\end{proof}}
\newcommand{\pf}{\begin{proof}}
\newcommand{\epf}{\end{proof}}


%New theorem definitions
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}
\newtheorem{corollary}{Corollary}
\newtheorem{conjecture}{Conjecture}
\newtheorem{lemma}{Lemma}
\newtheorem{proposition}{Proposition}
\newtheorem{assumption}{Assumption}

\newtheorem{model}{Model}
%
\theoremstyle{definition}
\newtheorem{definition}{Definition}
\newtheorem{example}{Example}
\newtheorem{remark}{Remark}
\newtheorem{remarks}{Remarks}



% Allows for custom theorem names
\newtheorem{innercustomthm}{Theorem} % Theorem
\newenvironment{customthm}[1]
  {\renewcommand\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}
\newtheorem{innercustomlem}{Lemma} % Lemma
\newenvironment{customlem}[1]
  {\renewcommand\theinnercustomlem{#1}\innercustomlem}
  {\endinnercustomthm}
\newtheorem{innercustomprop}{Proposition} % Proposition
\newenvironment{customprop}[1]
  {\renewcommand\theinnercustomprop{#1}\innercustomprop}
  {\endinnercustomthm}
\newtheorem{innercustomcor}{Corollary} % Corollary
\newenvironment{customcor}[1]
  {\renewcommand\theinnercustomcor{#1}\innercustomcor}
  {\endinnercustomthm}

